Qualitative Analysis and Adaptive Boosted DCA for Generalized Multi-Source Weber Problems

This paper has two primary objectives. First, we investigate fundamental qualitative properties of the generalized multi-source Weber problem formulated using the Minkowski gauge function. This includes proving the existence of global optimal solutions, demonstrating the compactness of the solution set, and establishing optimality conditions for these solutions. Second, we apply Nesterov's smoothing and the adaptive Boosted Difference of Convex functions Algorithm (BDCA) to solve both the unconstrained and constrained versions of the generalized multi-source Weber problems. These algorithms build upon the work presented in [6,19]. We conduct a comprehensive evaluation of the adaptive BDCA, comparing its performance to the method proposed in [19], and provide insights into its efficiency.

==> tables_in_example53.tex <==

\begin{table}[h]
	\centering
  \footnotesize
  \resizebox{0.9\textwidth}{!}{%
	\begin{tblr}
		{
		column{6} = {c},
		column{7} = {c},
		column{8} = {c},
		column{9} = {c},
		column{10} = {c},
		cell{1}{5} = {c=2}{},
		cell{1}{7} = {c=2}{},
		cell{1}{9} = {c=2}{},
		cell{2}{2} = {c},
		cell{2}{3} = {c},
		cell{2}{4} = {c},
		cell{2}{5} = {c},
		cell{3}{2} = {c},
		cell{3}{3} = {c},
		cell{3}{4} = {c},
		cell{3}{5} = {c},
		cell{4}{2} = {c},
		cell{4}{3} = {c},
		cell{4}{4} = {c},
		cell{4}{5} = {c},
		cell{5}{2} = {c},
		cell{5}{3} = {c},
		cell{5}{4} = {c},
		cell{5}{5} = {c},
		cell{6}{2} = {c},
		cell{6}{3} = {c},
		cell{6}{4} = {c},
		cell{6}{5} = {c},
		cell{7}{2} = {c},
		cell{7}{3} = {c},
		cell{7}{4} = {c},
		cell{7}{5} = {c},
		vline{7,9,11} = {1}{},
		vline{5-6,8,10} = {1}{},
				vline{2-11} = {2}{},
				vline{-} = {3-7}{},
				hline{1} = {5-10}{},
				hline{2} = {2-10}{},
				hline{3-8} = {-}{},
			}
		           &            &    &   & $\rho_F(x) = \|x\|_2$ &      & $\rho_F(x) = \|x\|_1$ &      & $\rho_F(x) = \|x\|_\infty$ &      \\
		           & m          & n  & k & {Iteration                                                                                      \\
		Ratio}     & {Time                                                                                                                 \\
		Ratio}     & {Iteration                                                                                                            \\
		Ratio~}    & {Time                                                                                                                 \\
		Ratio~}    & {Iteration                                                                                                            \\
		Ratio~}    & {Time                                                                                                                 \\
		Ratio~}                                                                                                                            \\
		Wine       & 178        & 13 & 3 & 1.31                  & 0.65 & 1.54                  & 0.73 & 1.41                       & 0.58 \\
		Iris       & 150        & 4  & 3 & 1.69                  & 0.79 & 1.61                  & 0.61 & 1.23                       & 0.56 \\
		PIMA       & 768        & 8  & 2 & 1.59                  & 0.79 & 1.36                  & 0.65 & 2.18                       & 0.96 \\
		Ionosphere & 351        & 34 & 2 & 1.42                  & 0.82 & 1.05                  & 0.46 & 1.40                       & 0.65 \\
		USCity     & 1217       & 2  & 3 & 3.93                  & 1.54 & 1.80                  & 0.53 & 2.07                       & 0.79
	\end{tblr}
 }
\caption{DCA/aBDCA ratios for time and iterations in \Cref{comparison tests} using \cref{BDCA unconstrained}}
	\label{table: 6 real datasets without skipping}
\end{table}

\begin{table}[h]
 \centering
 \footnotesize
 \resizebox{0.9\textwidth}{!}{%
	
	\begin{tblr}
		{
		column{6} = {c},
		column{7} = {c},
		column{8} = {c},
		column{9} = {c},
		column{10} = {c},
		cell{1}{5} = {c=2}{},
		cell{1}{7} = {c=2}{},
		cell{1}{9} = {c=2}{},
		cell{2}{2} = {c},
		cell{2}{3} = {c},
		cell{2}{4} = {c},
		cell{2}{5} = {c},
		cell{3}{2} = {c},
		cell{3}{3} = {c},
		cell{3}{4} = {c},
		cell{3}{5} = {c},
		cell{4}{2} = {c},
		cell{4}{3} = {c},
		cell{4}{4} = {c},
		cell{4}{5} = {c},
		cell{5}{2} = {c},
		cell{5}{3} = {c},
		cell{5}{4} = {c},
		cell{5}{5} = {c},
		cell{6}{2} = {c},
		cell{6}{3} = {c},
		cell{6}{4} = {c},
		cell{6}{5} = {c},
		cell{7}{2} = {c},
		cell{7}{3} = {c},
		cell{7}{4} = {c},
		cell{7}{5} = {c},
		vline{7,9,11} = {1}{},
		vline{5-6,8,10} = {1}{},
				vline{2-11} = {2}{},
				vline{-} = {3-7}{},
				hline{1} = {5-10}{},
				hline{2} = {2-10}{},
				hline{3-8} = {-}{},
			}
		           &            &    &   & $\rho_F(x) = \|x\|_2$ &      & $\rho_F(x) = \|x\|_1$ &      & $\rho_F(x) = \|x\|_\infty$ &      \\
		           & m          & n  & k & {Iteration                                                                                      \\
		Ratio}     & {Time                                                                                                                 \\
		Ratio}     & {Iteration                                                                                                            \\
		Ratio~}    & {Time                                                                                                                 \\
		Ratio~}    & {Iteration                                                                                                            \\
		Ratio~}    & {Time                                                                                                                 \\
		Ratio~}                                                                                                                            \\
		Wine       & 178        & 13 & 3 & 1.36                  & 1.27 & 1.51                  & 1.67 & 1.41                       & 1.27 \\
		Iris       & 150        & 4  & 3 & 1.75                  & 1.43 & 1.56                  & 1.20 & 1.31                       & 1.19 \\
		PIMA       & 768        & 8  & 2 & 2.02                  & 1.41 & 1.35                  & 1.13 & 2.09                       & 1.67 \\
		Ionosphere & 351        & 34 & 2 & 1.44                  & 1.32 & 1.09                  & 1.02 & 1.43                       & 1.33 \\
		USCity     & 1217       & 2  & 3 & 4.13                  & 3.71 & 1.77                  & 1.65 & 2.06                       & 1.91
	\end{tblr}
 }
\caption{DCA/aBDCA ratios for time and iterations in \Cref{comparison tests} using \cref{BDCA unconstrained - 2}}
	\label{table: 6 real datasets with skipping}
\end{table}
